Software Testing Meets Bayesian Workflow: A Literature-Driven Artifact Study of Probabilistic Programs

Automated testing is an effective software quality assurance method, but it is rarely used for probabilistic models. This is despite the heavy use of probabilistic programming for data analytics in research and engineering, where the consequences of errors are dire. A key obstacle is the specification of testable correctness properties for probabilistic models, known as the oracle problem. Like machine learning, probabilistic programming is used precisely where no analytical specification exists: had we been able to write one, we would have written an algorithm instead of fitting a model. An alternative is partial, proxy correctness specifications. The statistics literature already offers many, but as quality guidelines that require human judgment: comparing plots, visually analyzing shapes of distributions, assessing whether parameter values are ''far'' or ''close enough''. These guidelines are not systematically automated. In this work, we elicit, implement, and study testable correctness properties of probabilistic models. We extract 17 broadly applicable properties for probabilistic models from one of the most widely used textbooks in Bayesian data analysis, Statistical Rethinking by McElreath. For each property, we select and implement a test oracle, and study its utility for automatic testing, using a population of 59 probabilistic models from academic and industrial sources. We find realistic use cases (models under test) for all the properties. We observe that the vast majority of tests are not flaky in practice, despite the theoretical potential for flakiness. To the best of our knowledge, we are the first to investigate the effectiveness of mutation testing for probabilistic models, showing that standard mutation operators do not capture faults tracked by the probabilistic properties.

==> figures/error_vs_mutation_operator.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/error_vs_mutation_operator_fig.pdf}
    \caption{Error vs mutation operator}
    \label{fig:error_vs_operator}
\end{figure}

==> tables/flakiness_percentage.tex <==
\begin{table}[t!]
  \caption{Flakiness percentages based on model and property}
  \label{tab:flaky_precentages}
  \newcommand{\angleheader}{0}
  \begin{tabular}{
      l
      l
      p{1cm}
      p{1cm}
      p{1cm}
      p{1cm}
      p{1cm}
      p{1cm}
    }

    \toprule

    Property/Model &
    --- & 
    {\small Gsrm Latent Reg Itr} & 
    {\small Seeds Centered} & 
    {\small Normal MixtureK} & 
    {\small Eight School Centred} & 
    {\small State Space Stochastic Level Stochastic Seasonal}
    \\
    \midrule

    & 
    \begin{tabular}[c]{@{}l@{}}1-(flaky tests/\\ total tests)\end{tabular} & 
    0.50 & 
    0.67 & 
    0.67 & 
    0.75 & 
    0.50                                         
    \\

    KL-Divergence  & 
    0.84           & 
    0.42           & 
    0.56           & 
    0.56           &                    
    NA             &
    NA
    \\

    Unimodality & 
    0.92        &                  
    NA          &               
    NA          &                
    NA          & 
    0.69        & 
    0.46
    \\
    

    Skewness  & 
    0.93      &
    NA        &
    NA        &
    NA        &
    NA        & 
    0.47
    \\

    \bottomrule
  \end{tabular}
\end{table}


==> tables/flakiness_table.tex <==
\begin{table}[t!]
\caption{Practically flaky tests}
\label{tab:flaky}
\begin{tabular}{llll}

  \toprule

  Property & 
  Source & 
  Model &
  Pass/Fail 
  \\ 
  
  \midrule

  KL-Divergence & 
  PosteriorDB & 
  GrsmLatentRegIrt & 
  Fail      
  \\ 

  KL-Divergence & 
  PosteriorDB & 
  SeedsCenteredModel & 
  Fail      
  \\ 

  KL-Divergence & 
  PosteriorDB & 
  NormalMixtureKModel & 
  Pass      
  \\ 
  
  Unimodality   & 
  PosteriorDB & 
  EightSchoolsCenteredModel & 
  Pass      
  \\ 
  
  Unimodality   & 
  PosteriorDB & 
  StateSpaceStochasticLevelStochasticSeasonalModel & 
  Pass      
  \\ 
  
  Skewness & 
  PosteriorDB & 
  StateSpaceStochasticLevelStochasticSeasonalModel & 
  Pass      
  \\ 

  \bottomrule
\end{tabular}
\end{table}


==> tables/mutatation_operator_error_counts.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[h!]
\caption{Mutation operators least likely to cause errors, counts}
\label{tab:mutation_operator_count}
\begin{tabular}{lll}
\hline
Index & Mutation operator                       & \#mutations \\ \hline
1     & ReplaceBinaryOperator\_Mul\_BitAnd      & 76          \\
2     & ReplaceBinaryOperator\_Mul\_Add         & 76          \\
3     & ReplaceBinaryOperator\_Mul\_Mod         & 76          \\
4     & ReplaceBinaryOperator\_Mul\_Sub         & 73          \\
5     & ReplaceComparisonOperator\_Eq\_LtE      & 16          \\
6     & ReplaceComparisonOperator\_Eq\_Lt       & 16          \\
7     & ReplaceComparisonOperator\_Eq\_Gt       & 13          \\
8     & ReplaceComparisonOperator\_Eq\_NotEq    & 13          \\
9     & ReplaceComparisonOperator\_Eq\_GtE      & 12          \\
10    & AddNot                                  & 10          \\
11    & ReplaceBinaryOperator\_FloorDiv\_Mul    & 8           \\
12    & ReplaceBinaryOperator\_FloorDiv\_BitAnd & 8           \\
13    & ZeroIterationForLoop                    & 6           \\
14    & ReplaceBinaryOperator\_LShift\_Add      & 5           \\
15    & ReplaceComparisonOperator\_Gt\_NotEq    & 5           \\
16    & ReplaceComparisonOperator\_Gt\_Lt       & 4           \\
17    & ReplaceComparisonOperator\_Gt\_LtE      & 4           \\
18    & ReplaceComparisonOperator\_Gt\_GtE      & 4           \\
19    & ReplaceComparisonOperator\_Eq\_Is       & 3           \\
20    & ReplaceTrueWithFalse                    & 3          
\end{tabular}
\end{table}

==> tables/mutation_opreators.tex <==
\begin{table}[h!]
\caption{Mutation operators}
\label{tab:mutation}
\begin{tabular}{lll}
AddNot,                                  & ReplaceBinaryOperator\_FloorDiv\_Pow,    & ReplaceBinaryOperator\_RShift\_Mod,      \\
NumberReplacer,                          & ReplaceBinaryOperator\_FloorDiv\_RShift, & ReplaceBinaryOperator\_RShift\_Mul,      \\
RemoveDecorator,                         & ReplaceBinaryOperator\_FloorDiv\_Sub,    & ReplaceBinaryOperator\_RShift\_Pow,      \\
ReplaceBinaryOperator\_Add\_BitAnd,      & ReplaceBinaryOperator\_LShift\_Add,      & ReplaceBinaryOperator\_RShift\_Sub,      \\
ReplaceBinaryOperator\_Add\_BitOr,       & ReplaceBinaryOperator\_LShift\_BitAnd,   & ReplaceBinaryOperator\_Sub\_Add,         \\
ReplaceBinaryOperator\_Add\_BitXor,      & ReplaceBinaryOperator\_LShift\_BitOr,    & ReplaceBinaryOperator\_Sub\_BitAnd,      \\
ReplaceBinaryOperator\_Add\_Div,         & ReplaceBinaryOperator\_LShift\_BitXor,   & ReplaceBinaryOperator\_Sub\_BitOr,       \\
ReplaceBinaryOperator\_Add\_FloorDiv,    & ReplaceBinaryOperator\_LShift\_Div,      & ReplaceBinaryOperator\_Sub\_BitXor,      \\
ReplaceBinaryOperator\_Add\_LShift,      & ReplaceBinaryOperator\_LShift\_FloorDiv, & ReplaceBinaryOperator\_Sub\_Div,         \\
ReplaceBinaryOperator\_Add\_Mod,         & ReplaceBinaryOperator\_LShift\_Mod,      & ReplaceBinaryOperator\_Sub\_FloorDiv,    \\
ReplaceBinaryOperator\_Add\_Mul,         & ReplaceBinaryOperator\_LShift\_Mul,      & ReplaceBinaryOperator\_Sub\_LShift,      \\
ReplaceBinaryOperator\_Add\_Pow,         & ReplaceBinaryOperator\_LShift\_Pow,      & ReplaceBinaryOperator\_Sub\_Mod,         \\
ReplaceBinaryOperator\_Add\_RShift,      & ReplaceBinaryOperator\_LShift\_RShift,   & ReplaceBinaryOperator\_Sub\_Mul,         \\
ReplaceBinaryOperator\_Add\_Sub,         & ReplaceBinaryOperator\_LShift\_Sub,      & ReplaceBinaryOperator\_Sub\_Pow,         \\
ReplaceBinaryOperator\_BitAnd\_Add,      & ReplaceBinaryOperator\_Mod\_Add,         & ReplaceBinaryOperator\_Sub\_RShift,      \\
ReplaceBinaryOperator\_BitAnd\_BitOr,    & ReplaceBinaryOperator\_Mod\_BitAnd,      & ReplaceComparisonOperator\_Eq\_Gt,       \\
ReplaceBinaryOperator\_BitAnd\_Div,      & ReplaceBinaryOperator\_Mod\_BitOr,       & ReplaceComparisonOperator\_Eq\_GtE,      \\
ReplaceBinaryOperator\_BitAnd\_FloorDiv, & ReplaceBinaryOperator\_Mod\_BitXor,      & ReplaceComparisonOperator\_Eq\_Is,       \\
ReplaceBinaryOperator\_BitAnd\_LShift,   & ReplaceBinaryOperator\_Mod\_Div,         & ReplaceComparisonOperator\_Eq\_IsNot,    \\
ReplaceBinaryOperator\_BitAnd\_Mod,      & ReplaceBinaryOperator\_Mod\_FloorDiv,    & ReplaceComparisonOperator\_Eq\_Lt,       \\
ReplaceBinaryOperator\_BitAnd\_Mul,      & ReplaceBinaryOperator\_Mod\_LShift,      & ReplaceComparisonOperator\_Eq\_LtE,      \\
ReplaceBinaryOperator\_BitAnd\_Pow,      & ReplaceBinaryOperator\_Mod\_Mul,         & ReplaceComparisonOperator\_Eq\_NotEq,    \\
ReplaceBinaryOperator\_BitAnd\_RShift,   & ReplaceBinaryOperator\_Mod\_Pow,         & ReplaceComparisonOperator\_Gt\_Eq,       \\
ReplaceBinaryOperator\_BitAnd\_Sub,      & ReplaceBinaryOperator\_Mod\_RShift,      & ReplaceComparisonOperator\_Gt\_GtE,      \\
ReplaceBinaryOperator\_BitOr\_Add,       & ReplaceBinaryOperator\_Mod\_Sub,         & ReplaceComparisonOperator\_Gt\_Is,       \\
ReplaceBinaryOperator\_BitOr\_BitAnd,    & ReplaceBinaryOperator\_Mul\_Add,         & ReplaceComparisonOperator\_Gt\_IsNot,    \\
ReplaceBinaryOperator\_BitOr\_BitXor,    & ReplaceBinaryOperator\_Mul\_BitAnd,      & ReplaceComparisonOperator\_Gt\_Lt,       \\
ReplaceBinaryOperator\_BitOr\_Div,       & ReplaceBinaryOperator\_Mul\_BitOr,       & ReplaceComparisonOperator\_Gt\_LtE,      \\
ReplaceBinaryOperator\_BitOr\_FloorDiv,  & ReplaceBinaryOperator\_Mul\_BitXor,      & ReplaceComparisonOperator\_Gt\_NotEq,    \\
ReplaceBinaryOperator\_BitOr\_LShift,    & ReplaceBinaryOperator\_Mul\_Div,         & ReplaceComparisonOperator\_Lt\_Eq,       \\
ReplaceBinaryOperator\_BitOr\_Mod,       & ReplaceBinaryOperator\_Mul\_FloorDiv,    & ReplaceComparisonOperator\_Lt\_Gt,       \\
ReplaceBinaryOperator\_BitOr\_Mul,       & ReplaceBinaryOperator\_Mul\_LShift,      & ReplaceComparisonOperator\_Lt\_GtE,      \\
ReplaceBinaryOperator\_BitOr\_Pow,       & ReplaceBinaryOperator\_Mul\_Mod,         & ReplaceComparisonOperator\_Lt\_Is,       \\
ReplaceBinaryOperator\_BitOr\_RShift,    & ReplaceBinaryOperator\_Mul\_Pow,         & ReplaceComparisonOperator\_Lt\_IsNot,    \\
ReplaceBinaryOperator\_BitOr\_Sub,       & ReplaceBinaryOperator\_Mul\_RShift,      & ReplaceComparisonOperator\_Lt\_LtE,      \\
ReplaceBinaryOperator\_Div\_Add,         & ReplaceBinaryOperator\_Mul\_Sub,         & ReplaceComparisonOperator\_Lt\_NotEq,    \\
ReplaceBinaryOperator\_Div\_BitAnd,      & ReplaceBinaryOperator\_Pow\_Add,         & ReplaceComparisonOperator\_NotEq\_Eq,    \\
ReplaceBinaryOperator\_Div\_BitOr,       & ReplaceBinaryOperator\_Pow\_BitAnd,      & ReplaceComparisonOperator\_NotEq\_Gt,    \\
ReplaceBinaryOperator\_Div\_BitXor,      & ReplaceBinaryOperator\_Pow\_BitOr,       & ReplaceComparisonOperator\_NotEq\_GtE,   \\
ReplaceBinaryOperator\_Div\_FloorDiv,    & ReplaceBinaryOperator\_Pow\_BitXor,      & ReplaceComparisonOperator\_NotEq\_IsNot, \\
ReplaceBinaryOperator\_Div\_LShift,      & ReplaceBinaryOperator\_Pow\_Div,         & ReplaceComparisonOperator\_NotEq\_Lt,    \\
ReplaceBinaryOperator\_Div\_Mod,         & ReplaceBinaryOperator\_Pow\_FloorDiv,    & ReplaceComparisonOperator\_NotEq\_LtE,   \\
ReplaceBinaryOperator\_Div\_Mul,         & ReplaceBinaryOperator\_Pow\_LShift,      & ReplaceFalseWithTrue,                    \\
ReplaceBinaryOperator\_Div\_Pow,         & ReplaceBinaryOperator\_Pow\_Mod,         & ReplaceTrueWithFalse,                    \\
ReplaceBinaryOperator\_Div\_RShift,      & ReplaceBinaryOperator\_Pow\_Mul,         & ReplaceUnaryOperator\_Delete\_Invert,    \\
ReplaceBinaryOperator\_Div\_Sub,         & ReplaceBinaryOperator\_Pow\_RShift,      & ReplaceUnaryOperator\_Delete\_Not,       \\
ReplaceBinaryOperator\_FloorDiv\_Add,    & ReplaceBinaryOperator\_Pow\_Sub,         & ReplaceUnaryOperator\_Delete\_USub,      \\
ReplaceBinaryOperator\_FloorDiv\_BitAnd, & ReplaceBinaryOperator\_RShift\_Add,      & ReplaceUnaryOperator\_Invert\_Not,       \\
ReplaceBinaryOperator\_FloorDiv\_BitOr,  & ReplaceBinaryOperator\_RShift\_BitAnd,   & ReplaceUnaryOperator\_Invert\_USub,      \\
ReplaceBinaryOperator\_FloorDiv\_BitXor, & ReplaceBinaryOperator\_RShift\_BitOr,    & ReplaceUnaryOperator\_USub\_Invert,      \\
ReplaceBinaryOperator\_FloorDiv\_Div,    & ReplaceBinaryOperator\_RShift\_BitXor,   & ReplaceUnaryOperator\_USub\_Not,         \\
ReplaceBinaryOperator\_FloorDiv\_LShift, & ReplaceBinaryOperator\_RShift\_Div,      & ReplaceUnaryOperator\_USub\_UAdd,        \\
ReplaceBinaryOperator\_FloorDiv\_Mod,    & ReplaceBinaryOperator\_RShift\_FloorDiv, & ZeroIterationForLoop                     \\
ReplaceBinaryOperator\_FloorDiv\_Mul,    & ReplaceBinaryOperator\_RShift\_LShift,   &                                         
\end{tabular}
\end{table}

==> tables/mutation_opreators_2.tex <==
\begin{table}[h!]
\caption{Mutation operators}
\label{tab:mutation}
\begin{tabular}{lllll}
\hline
\multicolumn{1}{|l|}{-}                     & \multicolumn{1}{l|}{ReplaceBinaryOperator} & \multicolumn{1}{l|}{ReplaceBinaryOperator} & \multicolumn{1}{l|}{ReplaceComparisonOperator} & \multicolumn{1}{l|}{ReplaceUnaryOperator} \\ \hline
ReplaceFalseWithTrue,                       & Add\_BitAnd,                               & FloorDiv\_Pow,                             & Eq\_NotEq,                                     & Delete\_Invert,                           \\
ReplaceTrueWithFalse,                       & Add\_BitOr,                                & FloorDiv\_RShift,                          & Gt\_Eq,                                        & Delete\_Not,                              \\
ZeroIterationForLoop                        & Add\_BitXor,                               & FloorDiv\_Sub,                             & Gt\_GtE,                                       & Delete\_USub,                             \\
AddNot,                                     & Add\_Div,                                  & LShift\_Add,                               & Gt\_Is,                                        & Invert\_Not,                              \\
NumberReplacer,                             & Add\_FloorDiv,                             & LShift\_BitAnd,                            & Gt\_IsNot,                                     & Invert\_USub,                             \\
RemoveDecorator,                            & Add\_LShift,                               & LShift\_BitOr,                             & Gt\_Lt,                                        & USub\_Invert,                             \\ \cline{1-1}
\multicolumn{1}{|l|}{ReplaceBinaryOperator} & Add\_Mod,                                  & LShift\_BitXor,                            & Gt\_LtE,                                       & USub\_Not,                                \\ \cline{1-1}
Div\_Mod,                                   & Add\_Mul,                                  & LShift\_Div,                               & Gt\_NotEq,                                     & USub\_UAdd,                               \\
Div\_Mul,                                   & Add\_Pow,                                  & LShift\_FloorDiv,                          & Lt\_Eq,                                        &                                           \\
Div\_Pow,                                   & Add\_RShift,                               & LShift\_Mod,                               & Lt\_Gt,                                        &                                           \\
Div\_RShift,                                & Add\_Sub,                                  & LShift\_Mul,                               & Lt\_GtE,                                       &                                           \\
Div\_Sub,                                   & BitAnd\_Add,                               & LShift\_Pow,                               & Lt\_Is,                                        &                                           \\
FloorDiv\_Add,                              & BitAnd\_BitOr,                             & LShift\_RShift,                            & Lt\_IsNot,                                     &                                           \\
FloorDiv\_BitAnd,                           & BitAnd\_Div,                               & LShift\_Sub,                               & Lt\_LtE,                                       &                                           \\
FloorDiv\_BitOr,                            & BitAnd\_FloorDiv,                          & Mod\_Add,                                  & Lt\_NotEq,                                     &                                           \\
FloorDiv\_BitXor,                           & BitAnd\_LShift,                            & Mod\_BitAnd,                               & NotEq\_Eq,                                     &                                           \\
FloorDiv\_Div,                              & BitAnd\_Mod,                               & Mod\_BitOr,                                & NotEq\_Gt,                                     &                                           \\
FloorDiv\_LShift,                           & BitAnd\_Mul,                               & Mod\_BitXor,                               & NotEq\_GtE,                                    &                                           \\
FloorDiv\_Mod,                              & BitAnd\_Pow,                               & Mod\_Div,                                  & NotEq\_IsNot,                                  &                                           \\
FloorDiv\_Mul,                              & BitAnd\_RShift,                            & Mod\_FloorDiv,                             & NotEq\_Lt,                                     &                                           \\
Mod\_LShift,                                & BitAnd\_Sub,                               & Pow\_BitXor,                               & NotEq\_LtE,                                    &                                           \\
Mod\_Mul,                                   & BitOr\_Add,                                & Pow\_Div,                                  &                                                &                                           \\
Mod\_Pow,                                   & BitOr\_BitAnd,                             & Pow\_FloorDiv,                             &                                                &                                           \\
Mod\_RShift,                                & BitOr\_BitXor,                             & Pow\_LShift,                               &                                                &                                           \\
Mod\_Sub,                                   & BitOr\_Div,                                & Pow\_Mod,                                  &                                                &                                           \\
Mul\_Add,                                   & BitOr\_FloorDiv,                           & Pow\_Mul,                                  &                                                &                                           \\
Mul\_BitAnd,                                & BitOr\_LShift,                             & Pow\_RShift,                               &                                                &                                           \\
Mul\_BitOr,                                 & BitOr\_Mod,                                & Pow\_Sub,                                  &                                                &                                           \\
Mul\_BitXor,                                & BitOr\_Mul,                                & RShift\_Add,                               &                                                &                                           \\
Mul\_Div,                                   & BitOr\_Pow,                                & RShift\_BitAnd,                            &                                                &                                           \\
Mul\_FloorDiv,                              & BitOr\_RShift,                             & RShift\_BitOr,                             &                                                &                                           \\
Mul\_LShift,                                & BitOr\_Sub,                                & RShift\_BitXor,                            &                                                &                                           \\
Mul\_Mod,                                   & Div\_Add,                                  & RShift\_Div,                               &                                                &                                           \\
Mul\_Pow,                                   & Div\_BitAnd,                               & RShift\_FloorDiv,                          &                                                &                                           \\
Mul\_RShift,                                & Div\_BitOr,                                & RShift\_LShift,                            &                                                &                                           \\
Mul\_Sub,                                   & Div\_BitXor,                               & Pow\_BitAnd,                               &                                                &                                           \\
Pow\_Add,                                   & Div\_FloorDiv,                             & Pow\_BitOr,                                &                                                &                                           \\
Div\_LShift,                                &                                            &                                            &                                                &                                          
\end{tabular}
\end{table}

==> tables/properties_vs_models.tex <==
\begin{table}[t]

  \renewcommand \arraystretch {0.9}

  \begin{tabular}{
    >{\small}l
    >{\small}c
    >{\small}c
    >{\small}c
  }

    \textbf{Property}                            & \textbf{PyMC docs}     & \textbf{SR}             & \textbf{PosteriorDB}    \\
    \midrule
    Categorical Variable Validation                            & 1                      & 2                       & 0                       \\
    Correlation matrix values             & 0                      & 1                       & 0                       \\
    Conditional Independence                            & 0                      & 1                       & 1                       \\
    K-1 model completeness               & 0                      & 2                       & 1                       \\
    Information Content of the Likelihood                         & 1                      & 0                       & 7                       \\
    Link-function Match                  & 1                      & 4                       & 0                       \\
    Multicollinearity                        & 0                      & 1                       & 9                       \\
    Non-Centered Parameterization       & 0                      & 0                       & 0                       \\
    Data-Distribution match                 & 0                      & 4                       & 3                       \\
    test\_over\_dispertion\_varaince\_compliance & 0                      & 4                       & 0                       \\
    test\_parameter\_reconstruction              & 2                      & 0                       & 0                       \\
    test\_prior\_flatness                        & 0                      & 1                       & 0                       \\
    test\_scientific\_validity                   & 0                      & 2                       & 0                       \\
    test\_shrinkage\_validation                  & 1                      & 0                       & 2                       \\
    test\_skewness                               & 0                      & 1                       & 6                       \\
    test\_unimodality                            & 0                      & 1                       & 5                       \\
    test\_zero\_inflation                        & 0                      & 1                       & 0                       \\
    \midrule
    Sum                                          & 6                      & 25                      & 34                      \\
    \bottomrule
  \end{tabular}

  \medskip

  \caption {Tests, 65 property-model pairs, used in \cref{sec:eval:rq3}, all pass and are not practically flaky (\cref{sec:eval:rq2}).}%
  \label{tab:properties_vs_models}

  \vspace {-3ex plus 3pt minus 1pt}

\end{table}

